A Simplified Gravitational Reference Sensor for Satellite Geodesy

We describe a Simplified Gravitational Reference Sensor (S-GRS), an ultra-precise inertial sensor for future Earth geodesy missions. These sensors are used to measure or compensate for all non-gravitational accelerations of the host spacecraft so that they can be removed in the data analysis to recover spacecraft motion due to Earth's gravity field, which is the main science observable. Low-low satellite-to-satellite tracking missions like GRACE-FO that utilize laser ranging interferometers are technologically limited by the acceleration noise performance of their electrostatic accelerometers, in addition to temporal aliasing associated with Earth's dynamic gravity field. The S-GRS is estimated to be at least 40 times more sensitive than the GRACE accelerometers and more than 500 times more sensitive if operated on a drag-compensated platform. The improved performance is enabled by increasing the mass of the sensor's test mass, increasing the gap between the test mass and its electrode housing, removing the small grounding wire used in the GRACE accelerometers and replacing them with a UV LED-based charge management system. This level of improvement allows future missions to fully take advantage of the sensitivity of the GRACE-FO laser Ranging Interferometer in the gravity recovery analysis. The S-GRS concept is a simplified version of the flight-proven LISA Pathfinder GRS. Our performance estimates are based on models vetted during the LISA Pathfinder flight and the expected Earth orbiting spacecraft environment based on flight data from GRACE-FO. The relatively low volume, mass, and a power consumption enables use of the S-GRS on ESPA-class microsatellites, reducing launch costs or enabling larger numbers of satellite pairs to be utilized to improve the temporal resolution of Earth gravity field maps.

==> old_bib.tex <==
% Non-BibTeX users please use
\begin{thebibliography}{}
%
% and use \bibitem to create references. Consult the Instructions
% for authors for reference list style.
%
%\bibitem{RefJ}
% Format for Journal Reference
%Author, Article title, Journal, Volume, page numbers (year)
% Format for books
%\bibitem{RefB}
%Author, Book title, page numbers. Publisher, place (year)
% etc

\bibitem{abich2019}
Abich K et al (2019) In-orbit performance of the GRACE Follow-On Laser Ranging Interferometer. Phys Rev Lett 123:031101

\bibitem{abich2015}
Abich K et al (2015) GRACE-Follow On Laser Ranging Interferometer: German contribution. J  Phys Conf Ser 610:012010

% \textcolor{red}{Not in text:} Antonucci, F., et al. (2011). LISA Pathfinder: mission and status, Classical and Quantum Gravity, Vol. 28, No. 9, 094001.

\bibitem{armano2018}
Armano M et al (2018) Beyond the Required LISA Free-Fall Performance: New LISA Pathfinder Results down to 20\,$\mu$Hz. Phys Rev Lett 120(6):061101,  doi: 10.1103/PhysRevLett.120.061101

\bibitem{bortoluzzi2012}
Bortoluzzi D, Zanoni C, Conklin JW (2012) Prediction of the LISA-Pathfinder release mechanism in-flight performance. Adv Space Res 51:1145-1156 

\bibitem{bortoluzzi2016}
Bortoluzzi D, Armano M, Audley, H, et al (2016). Injection of a Body into a Geodesic: Lessons Learnt from the LISA Pathfinder Case. NASA Aerospace Mechanisms Symposium 43:15-28

\bibitem{carbone2007}
Carbone L, Cavalleri A, Ciani G, Dolesi R, Hueller M, Tombolato D, Vitale S, Weber WJ (2007) Thermal gradient-induced forces on geodesic reference masses for LISA. Phys. Rev. D 76(10):102003, doi: 10.1103/PhysRevD.76.102003

\bibitem{christophe2010}
Christophe B, Marque J-P, Foulon B (2010) In-orbit data verification of the accelerometers of the ESA GOCE mission. SF2A-2010: Proceedings of the Annual meeting of the French Society of Astronomy and Astrophysics, pp 113-116

% \textcolor{red}{Not in text:} Christophe, B., Liorzou, F., Lebat, V., Boulanget, D., Dalin, M., Hardy, E., Zahzam, N., Bresson, A., Bibel, Y. (2019) ONERA accelerometers for future gravity mission, Fall AGU Meeting 2019, Poster G51B-0594.

\bibitem{ciani2008}
Ciani G (2008) Free-fall of LISA Test Masses: a new torsion pendulum to test translational acceleration.Doctoral dissertation, University of Trento pp 16

\bibitem{ciani2017}
Ciani G, Aitken M, Apple S, Chilton A, Olatunde T, Mueller G, Conklin JW  (2017) A New Torsion Pendulum for Gravitational Reference Sensor Technology Development. Rev Sci Instrum 88(6):064502

\bibitem{dahl2016}
Dahl C, Baatzsch A, Dehne M, Gilles F, Hager P, Herding M, Nicklaus K, Voss K, Abich K, Braxmaier C, Gohlke M, Guenther B, Sanjuan J, Zender B, Barranco G F, Görth A, Mahrdt C, Müller V, Schütze D, Stede G, Heinzel G (2016) Laser ranging interferometer on Grace follow-on. Proc. SPIE 10562, International Conference on Space Optics — ICSO 2016, 105623V, doi:10.1117/12.2297705

% \bibitem[(Danzmann 2003)]{LISA}
\bibitem{LISA}
Danzmann~K, Rudiger~A (2003) LISA technology: concept, status, prospects.
Class Quantum Gravity 20:S1-S9, doi: 10.1088/0264-9381/20/10/301

\bibitem{daras2018}
Daras I, and Pail R (2017) Treatment of temporal aliasing effects in the context of next generation satellite gravimetry missions. J Geophys Res Solid Earth 122:7343-7362, doi:10.1002/2017JB014250. 

% \textcolor{red}{Not in text:}  Dionisio, s., Anselmi, A., Bonino, L., Cesare, S., Massotti, L., Silvestrin, P. (2018) The “Next Generation Gravity Mission” challenges, consolidation of the system concepts and technological innovations, Proceedings of the 2018 SpaceOps Conference, doi:10.2514/6.2018-2495.

% \textcolor{red}{Not in text:} Elliott, E.R., Krutzik, M.C., Williams, J.R., Thompson, R.J., Aveline, D.C. (2018). NASA’s Cold Atom Lab (CAL): system development and ground test status, NPJ Microgravity, Vol. 4, No. 16, doi:10.1038/s41526-018-0049-9.

% \bibitem[(Dolesi 2003)]{LPF_GRS}
\bibitem{LPF_GRS}
Dolesi~R, Bortoluzzi~D, Bosetti~P, Carbone~L, Cavalleri~A,
Cristofolini~I, DaLio~M, Fontana~G, Fontanari~V, Foulon~B,
Hoyle~CD, Hueller~M, Nappo~F, Sarra~P, Shaul~DNA, Sumner~T,
Weber~WJ, Vitale~S (2003)
Gravitational sensor for LISA and its technology
demonstration mission
Class Quant Grav
20:S99â€“S108. doi: 10.1088/0264-9381/20/10/312


% \bibitem[(Drinkwater 2003)]{GOCE}
\bibitem{GOCE}
Drinkwater~MR, Floberghagen~R, Haagmans~R, Muzi~D, Popescu~A (2003)
GOCE: ESA's First Earth Explorer Core Mission.
Space Sci S 17:419-432, doi: 10.1023/A:1026104216284

\bibitem{elsaka2013}
Elsaka B, Raimondo JC, Brieden P, Reubelt T, Kusche J, Flechtner F, Pour SI, Sneeuw N, Muller J (2013) Comparing seven candidate mission configurations for temporal gravity field retrieval through full-scale numerical simulation. J Geod 88:31-43, doi: 10.1007/s00190-013-0665-9

% \bibitem[(Everitt 2011)]{prl}
\bibitem{prl}
Everitt~CWF, Debra~DB, Parkinson~BW, Turneaure~JP, Conklin~JW, Heifetz~MI,
Keiser~GM, Silbergleit~AS, Holmes, T, Kolodziejczak J, Al-Meshari~M,
Mester~JC, Muhlfelder~B, Solomonik~VG, Stahl~K, Worden~PW Jr, Bencze~W,
Buchman~S, Clarke~B, Al-Jadaan~A, Al-Jibreen~H, Li~J, Lipa~JA, Lockhart~J~M,
Al-Suwaidan~B, Taber~M, Wang~S (2011) 
Gravity Probe~B: Final Results of a Space Experiment to Test General
Relativity.
Phys Rev Lett
106:221101-1. doi: 10.1103/PhysRevLett.106.221101

\bibitem{fleddermann2014}
Fleddermann R, Ward RL, Elliot M, Wuchenich DM, Gilles F, Herding M, Nicklaus K, Brown J, Burke J, Dligatch S, Farrant DI, Green KL, Seckold JA, Blundell M, Brister R, Smith C, Sheard BS, Heinzel G, Danzmann K, Klipstein B, McClelland DE, Shaddock SA (2014). Testing the GRACE follow-on triple mirror assembly. Class Quantum Gravity 31:195004. doi:10.1088/0264-9381/31/19/195004

\bibitem{gerardi2014}
Gerardi D, Allen G, Conklin, JW, Sun KX, DeBra D, Buchman S, Gath P, Fichter W, Byer RL, Johann U (2014) Invited Article: Advanced drag-free concepts for future space-based interferometers: acceleration noise performance. Rev Sci Instrum 85(1):011301

\bibitem{ghobadi2018}
Ghobadi-Far K, Han S-C, Weller S, Loomis BD, Luthcke SB, Mayer-Gurr T, Behzadpour S (2018) A Transfer function between line-of-sight gravity difference and GRACE intersatellite ranging data and an application to hydrological surface mass variation. J Geophys Res Solid Earth 123:9186-9201, doi.org/10.1029/2018JB016088. 

\bibitem{ghobadi2020}
Ghobadi-Far K, Han S-C, McCullough C, DWiese DN, Yuan D-N, Landerer FW, Sauber J, Watkins MM (2020) GRACE Follow-On Laser Ranging Interferometer Measurements Uniquely Distinguish Short-Wavelength Gravitational Perturbations. Geophys Res Lett 47 e2020GL089445, doi.org/10.1029/2020GL089445.

\bibitem{halloin2013}
Halloin H, Prat P, Brossard J (2013) Long term characterization of voltage references. ArXiv:1312.5101v1

\bibitem{hauk2020}
Hauk M, Wiese DN (2020) New methods for linking science objectives to remote sensing observations: a concept study using single- and dual-pair satellite gravimetry architectures. Earth Space Sci 7 e2019EA000922, doi.org/10.1029/2019EA000922.

\bibitem{inchauspe2020}
Inchausp{\'e} H, Olatunde T, Apple S, Parry S, Letson B, Mueller G, Wass P, Conklin JW (2020) Numerical Modeling and Experimental Demonstration of Pulsed Charge Control for the Space Inertial Sensor used in LISA. Phys Rev D 102(4):042002

%JPL (2018). https://gracefo.jpl.nasa.gov/interactives/spacecraft/

\bibitem{josselin1999}
Josselin V, Touboul P, Kielbasa R (1999) Capacitive detection scheme for space accelerometers applications. Sensors and Actuators 78:92–98 

\bibitem{kersevan2009}
Kersevan R, Pons J-L (2009). Introduction to MOLFLOW+: New graphical processing unit-based Monte Carlo code for simulating molecular flows and for calculating angular coefficients in the compute unified device architecture environment. J Vac Sci Technol 27:1017-023, doi.org/10.1116/1.3153280.

% \textcolor{red}{Not in text:} Lebat, V., Boulanger, D., Christophe, B., Foulon, B., Liorzou, F., Perrot, E. (2013). Electrostatic accelerometer for the Gravity Recovery and Climate Experiment Follow-On Mission (GRACE-FO), Fall AGU Meeting 2013, Poster G33B-0989. 

\bibitem{lotters1999}
L\"otters JC, Olthuis W, Veltink PH, Bergveld P (1999) A sensitive differential capacitance to voltage converter for sensor applications. 	IEEE T Instrum Meas 48:89-96 

\bibitem{martin2015} Mateos-Martin JI (2015) Design and assessment of a low-frequency magnetic measurement system for eLISA. Thesis 

\bibitem{MC2020a}
Mass Change Study Team (2020a) Mass Change Designated Observable Science and Applications Traceability Matrix, https://science.nasa.gov/earth-science/decadal-mc.

\bibitem{MC2020b}
Mass Change Study Team (2020b) The NASA Mass Change Designated Observable Study AGU 2020 Town Hall, https://science.nasa.gov/earth-science/decadal-mc.

\bibitem{mcnamara2013}
McNamara P, Antonucci F, Armano M, et al (2013) The LISA Pathfinder Mission, ASP Conference Series 467:5-16

\bibitem{mehta2017}
Mehta PM, Walker AC, Sutton EK, Godinez HC (2017) New density estimates derived using accelerometers on board the CHAMP and GRACE satellites, Space Weather 15:558–576 doi:10.1002/2016SW001562.

\bibitem{miarnau2015}
Miarnau A, Schneider G, Veness R (2015) Development and test of a rectangular CERN ConFlat-type flange, Vacuum 121:202-206 doi:10.1016/j.vacuum.2015.08.018.

\bibitem{montenbruck2000}
Montenbruck O, Gill E (2000) Satellite Orbits. Springer, New York, NY, pp 89-91

\bibitem{GEVS}
NASA Goddard Space Flight Center (2018) General Environmental Verification Standard (GEVS), GSFC-STD-7000, Rev. A, https://standards.nasa.gov/standard/gsfc/gsfc-std-7000.

\bibitem{natacad2018}
National Academies of Sciences, Engineering, and Medicine (2018) Thriving on Our Changing Planet: A Decadal Strategy for Earth Observation from Space., Washington DC: The National Academies Press., https://doi.org/10.17226/24938. 

\bibitem{olatunde2015}
Olatunde T, Shelley R, Chilton A, Ciani G, Mueller G, Conklin JW (2015) 240 nm UV LEDs for LISA test mass charge control. Proceedings of the 10th International LISA Symposium, J Phys Conf Ser 610(1):012034

\bibitem{pail2015}
Pail R, Bingham R, Braitenberg C, Dobslaw H, Eicker A, Guntner A, Horwath M, Ivins E, Longueverne L, Panet I, Wouters B, IUGG Expert Panel (2015) Science and user needs for observing global mass transport to understand global change and to benefit society. Survey of Geophysics 36:743-772, doi:10.1007/s10712-015-9348-9. 

\bibitem{peidou2021}
Peidou A, Landerer F, Wiese DN, Ellmer M, Fahnestock E, McCullough C, Spero R, Yuan D-N (2021), Spatiotemporal characterization of geophysical signal detection capabilities of GRACE-FO. Submitted to Geophys Res Lett
% \bibitem[(Reigber 2002)]{CHAMP}
\bibitem{CHAMP}
Reigber~Ch, L\"uhr~H, Schwintzer~P (2002)
CHAMP mission status.
Adv Space Res 30:129-134, doi: 10.1016/S0273-1177(02)00276-4

% \bibitem[(Sheard 2012)]{GRACE-FO}
\bibitem{GRACE-FO}
Sheard~BS, Heinzel~G, Danzmann~K, Shaddock~DA, Klipstein~WM, Folkner~WM
(2012)
Intersatellite laser ranging instrument for the GRACE
follow-on mission.
J Geod
86:1083-1095, doi: 10.1007/s00190-012-0566-3

\bibitem{speake1997}
Speake CC, Andrews PL (1997) Capacitive sensing for drag-free satellites. Class Quantum Gravity 14:1557-1565

\bibitem{spero2021}
Spero R (2021) Point-mass sensitivity of gravimetric satellites. Adv Space Res 67(5):1656-1664 

% \bibitem[(Tapley 2004)]{GRACE}
\bibitem{GRACE}
Tapley~BD, Bettadpur~S, Watkins~M and Reigber~C (2004)
The gravity recovery and climate experiment: Mission overview and early results. Geophys Res Lett
31:L09607, doi: 10.1029/2004GL019920

\bibitem{tapley2019} Tapley BD, Watkins MM, Flechtner F et al (2019) Contributions of GRACE to Understanding Climate Change. Nature Climate Change, 9:358-369, doi:10.1038/s41558-019-0456-2

\bibitem{touboul1999}
Touboul P, Foulon B, and Willemenot (1999) Electrostatic space accelerometers for present and future missions. Acta Astronautica, 45(10):605–617.

% \bibitem[(Touboul 2001)]{microscope}
\bibitem{microscope}
Touboul~P, Rodrigues~M, M{\'e}tris~G, Tatry~B (2001)
MICROSCOPE, testing the equivalence principle in space.
Cr Acad Sci IV-Phys
2:1271-86. doi: 10.1016/S1296-2147(01)01264-1

% \textcolor{red}{Not in text:} Thompson, R., Folkner, W.M., deVine, G., Klipstein, W.M., McKenzie, K., Spero, R., Yu, N., Stephens, M., Leitch, J., Pierce, R. (2011) A Flight-Like Optical Reference Cavity for GRACE Follow-on Laser Frequency Stabilization, IEEE International Frequency Control Symposium, 729-731, ISBN 978-1-61284-110-6. 

\bibitem{wass2018}
Wass PJ, and the LISA Pathfinder Collaboration (2018) Precision charge control for isolated free-falling test masses: LISA pathfinder results, Phys Rev D 98:062001 

\bibitem{weber2002}
Weber WJ, Cavalleri A, Dolesi R et al (2002) Position sensors for LISA drag-free control. Class Quantum Gravity 19:1751-1756 

\bibitem{wiese2012}
Wiese DN, Nerem RS, Lemoine FG (2012) Design considerations for a dedicated gravity recovery satellite mission consisting of two pairs of satellites. J Geod 86:81—98 doi: 10.1007/s00190-011-0493-8

\bibitem{wiese2011a}
Wiese DN, Nerem RS, Han SC (2011) Expected Improvements in Determining Continental Hydrology, Ice Mass Variations, Ocean Bottom Pressure Signals, and Earthquakes using Two Pairs of Dedicated Satellites, for Temporal Gravity Recovery. J Geophys Res Solid Earth 116:B11405, doi:10.1029/2011JB008375

\bibitem{wiese2011b}
Wiese  DN, Visser P, Nerem, RS (2011) Estimating Low Resolution Gravity Fields at Short Time Intervals to Reduce Temporal Aliasing Errors. Adv Space Res 48:1094-1107, doi: 10.1016/j.asr.2011.05.027.

\end{thebibliography}
